Deep Clustering of Text Representations for Supervision-free Probing of Syntax

We explore deep clustering of text representations for unsupervised model interpretation and induction of syntax. As these representations are high-dimensional, out-of-the-box methods like KMeans do not work well. Thus, our approach jointly transforms the representations into a lower-dimensional cluster-friendly space and clusters them. We consider two notions of syntax: Part of speech Induction (POSI) and constituency labelling (CoLab) in this work. Interestingly, we find that Multilingual BERT (mBERT) contains surprising amount of syntactic knowledge of English; possibly even as much as English BERT (EBERT). Our model can be used as a supervision-free probe which is arguably a less-biased way of probing. We find that unsupervised probes show benefits from higher layers as compared to supervised probes. We further note that our unsupervised probe utilizes EBERT and mBERT representations differently, especially for POSI. We validate the efficacy of our probe by demonstrating its capabilities as an unsupervised syntax induction technique. Our probe works well for both syntactic formalisms by simply adapting the input representations. We report competitive performance of our probe on 45-tag English POSI, state-of-the-art performance on 12-tag POSI across 10 languages, and competitive results on CoLab. We also perform zero-shot syntax induction on resource impoverished languages and report strong results.

==> sections/6-discussion.tex <==
\section{Discussion: Clustering Multilingual BERT Representations}
~\cite{pires2019multilingual} 
\begin{itemize}
\item 
did show mBERT’s ability to transfer between languages that are written in different scripts, and thus have effectively zero lexical overlap. There were results (e.g. Figure 1) showing that while performance using EN-BERT depends directly on word piece overlap, mBERT’s performance is largely independent of overlap, indicating that it learns multilingual representations deeper than simple vocabulary memorization.
\item 
As to why mBERT generalizes across languages, we hypothesize that having word pieces used in all languages (numbers, URLs, etc) which have to be mapped to a shared space forces the co-occurring pieces to also be mapped to a shared space, thus spreading the effect to other word pieces, until different languages are close to a shared space.
\item 
In each of these three dimensions, the authors run experiments to test why BERT is effective at cross-lingual transfer.
For simplicity, they run their experiments on B-BERT which is trained on two languages. The fine-tuning is done on language, and the zero-shot performance is tested on the other one.
\item 
Among the most surprising results, an mBERT model that has been fine-tuned using only POS- labeled Urdu (written in Arabic script), achieves 91\% accuracy on Hindi (written in Devanagari script), even though it has never seen a single POS- tagged Devanagari word. This provides clear evidence of \mbert’s multilingual representation ability, mapping structures onto new vocabularies based on a shared representation induced solely from monolingual language model training data.
\item
However, cross-script transfer is less accurate for other pairs, such as English and Japanese, indi- cating that mBERT’s multilingual representation is not able to generalize equally well in all cases.
A possible explanation for this, as we will see in section 4.2, is typological similarity. English and Japanese have a different order of subject, verb and object, while English and Bulgarian have the same, and mBERT may be having trouble generalizing across different orderings.
\end{itemize}

==> sections/extra.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |l|c|c| } 
\hline
Method & M1 & VM\\
\hline
\syntdecmorph & 78.3 ($\pm$0.7) & 72.8 ($\pm$0.5)\\
\syntdec & 76.6 ($\pm$1.5) & 71.5 ($\pm$0.9)\\
\sae & 74.3 ($\pm$1.4) & 68.9 ($\pm$0.9)\\
\kmeansmethod & 71.4 ($\pm$2.9)  & - \\
\hline
%Baum-Welch & 62.6 ($\pm$1.1)  & -\\
\citet{brown1992class} & 65.6 ($\pm$NA) & -\\
\citet{stratos2016unsupervised} & 67.7 ($\pm$NA) & -\\
\citet{berg2010painless} & 74.9 ($\pm$1.5) & -\\ 
\citet{blunsom2011hierarchical} & 77.5($\pm$NA) & 69.8\\ 
\citet{stratos2018mutual} & 78.1 ($\pm$0.8) & -\\ 
\hline
\hline
\citet{tran2016unsupervised} (*) & 79.1 & 71.7\\
\syntdecbest & 79.7 & 73.6 \\
\hline
\hline
\citet{yuret2014unsupervised} (token-based) & 79.5  & 69.1 \\
\citet{yatbaz2012learning} (word-based) & 80.2  & 72.1 \\
\citet{he2018unsupervised} (*) & 80.8 ($\pm$1.3) & 74.1 ($\pm$0.7)\\
\syntdecmorphparsed & 79.5 ($\pm$0.9) & 73.9 ($\pm$0.7)\\
\hline
\end{tabular}
}
\caption{Many-to-one (M1) accuracy and V-Measure (VM) of \posi on the 45-tag Penn Treebank WSJ dataset for 10 random runs. \mbert is used in all of our experiments (upper part of the table). (*): See text for discussion. \cite{y}
}
\label{table:1}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[t]
\begin{subtable}[h]{\columnwidth}
\resizebox{\columnwidth}{!}{

\centering
\begin{tabular}{|l|c|c|}
\hline
Method & M1 & VM\\
\hline
\syntdecmorph & 78.3 ($\pm$0.7) & 72.8 ($\pm$0.5)\\
\syntdec & 76.6 ($\pm$1.5) & 71.5 ($\pm$0.9)\\
\sae & 74.3 ($\pm$1.4) & 68.9 ($\pm$0.9)\\
\kmeansmethod & 71.4 ($\pm$2.9)  & - \\
\hline
\citet{brown1992class} & 65.6 ($\pm$NA) & -\\
\citet{stratos2016unsupervised} & 67.7 ($\pm$NA) & -\\
\citet{berg2010painless} & 74.9 ($\pm$1.5) & -\\ 
\citet{blunsom2011hierarchical} & 77.5($\pm$NA) & 69.8\\ 
\citet{stratos2018mutual} & 78.1 ($\pm$0.8) & -\\ 
\citet{tran2016unsupervised} (*) & 79.1 ($\pm$NA) & 71.7 ($\pm$NA)\\
%\syntdecbest & 79.7 & 73.6 \\
\hline
\end{tabular}
}
\caption{Tagged data}
\label{tab:week1}

\end{subtable}
\hfill
\begin{subtable}[h]{\columnwidth}
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{|l|c|c|}
\hline
\citet{yuret2014unsupervised} (token-based) & 79.5  & 69.1 \\
\citet{yatbaz2012learning} (word-based) & 80.2  & 72.1 \\
\citet{he2018unsupervised} (*) & 80.8 ($\pm$1.3) & 74.1 ($\pm$0.7)\\
\syntdecmorphparsed & 79.5 ($\pm$0.9) & 73.9 ($\pm$0.7)\\
\hline
\end{tabular}
}
\caption{Parsed data}
\label{tab:week2}
\end{subtable}
\caption{Many-to-one (M1) accuracy and V-Measure (VM) of \posi on the 45-tag Penn Treebank WSJ dataset for 10 random runs. \mbert is used in all of our experiments (upper part of the table). (*): See text for discussion.}
\label{tab:temps}
\end{table}
\end{comment}

